Separations of Matroid Freeness Properties

Properties of Boolean functions on the hypercube invariant with respect to linear transformations of the domain are among the most well-studied properties in the context of property testing. In this paper, we study the fundamental class of linear-invariant properties called matroid freeness properties. These properties have been conjectured to essentially coincide with all testable linear-invariant properties, and a recent sequence of works has established testability for increasingly larger subclasses. One question left open, however, is whether the infinitely many syntactically different properties recently shown testable in fact correspond to new, semantically distinct ones. This is a crucial issue since it has also been shown that there exist subclasses of these properties for which an infinite set of syntactically different representations collapse into one of a small, finite set of properties, all previously known to be testable. An important question is therefore to understand the semantics of matroid freeness properties, and in particular when two syntactically different properties are truly distinct. We shed light on this problem by developing a method for determining the relation between two matroid freeness properties P and Q. Furthermore, we show that there is a natural subclass of matroid freeness properties such that for any two properties P and Q from this subclass, a strong dichotomy must hold: either P is contained in Q or the two properties are "well separated." As an application of this method, we exhibit new, infinite hierarchies of testable matroid freeness properties such that at each level of the hierarchy, there are functions that are far from all functions lying in lower levels of the hierarchy. Our key technical tool is an apparently new notion of maps between linear matroids, called matroid homomorphisms, that might be of independent interest.

==> acknowledgements.tex <==
\section*{Acknowledgments}

%    
%    We are greatly indebted to Madhu Sudan for raising the questions
%    addressed in this paper as well as numerous insights, suggestions and
%    comments.  We also thank Asaf Shapira for his collaboration at the
%    beginning stages of the research as well as his useful advice
%    throughout.
%    

We are grateful to Madhu Sudan for suggesting that we investigate the
problems studied in this work,  for giving many helpful insights and comments
along the way,  and for challenging us to redouble our efforts  in
order to strengthen our first, preliminary results. 
We also want to thank Asaf Shapira for his collaboration in the early
stages of this research, as well as for his continuing useful advice.



==> definitions-article.tex <==
%
% MISCELLANEOUS DEFINITIONS TO USE IN LaTeX-FILES
%-------------------------------------------------
%
% Last updated 08-01-14
%

%
% Stuff specific for the ``article'' article class.
%

%
% EQUATIONS, THEOREMS, PROOFS AND SUCH
%
% Requires \usepackage{amstex} or \usepackage{amsmath}
% Requires \usepackage{theorem}
% Requires \usepackage{ifthen}
%

%
% To get equation numbered within sections, e.g. (3.2) for the 2nd
% equation in section 3, use \numberwithin
%\numberwithin{equation}{section}
%
% To get a cross-reference to an equation with parantheses, use
% \eqref{}
%
% To get ``subequations'' numbered e.g. (4.9a), (4.9b), use
% \begin{subequations}
%       equations to be numbered
% \end{subequations}
%

%
% NOTE THAT \theoremheaderfont{} IS A *GLOBAL* DECLARATION!
%

% number all theorem structures using ``standardlocalcounter'' 
% with consecutive numbers
\newtheorem{standardlocalcounter}{Dummy}[section]
\newtheorem{standardglobalcounter}{Dummy}

% insert a linebreak between theorem head and body
\theoremstyle{plain}    

\newtheorem{theorem}[standardlocalcounter]{Theorem}
\newtheorem{lemma}[standardlocalcounter]{Lemma}
\newtheorem{proposition}[standardlocalcounter]{Proposition}
\newtheorem{corollary}[standardlocalcounter]{Corollary}
\newtheorem{observation}[standardlocalcounter]{Observation}
\newtheorem{fact}[standardlocalcounter]{Fact}

\newtheorem{conjecturelocalcounter}[standardlocalcounter]{Conjecture}
\newtheorem{conjectureglobalcounter}[standardglobalcounter]{Conjecture}
\newtheorem{conjecture}[standardglobalcounter]{Conjecture}
\newtheorem{openquestion}[standardglobalcounter]{Open Question}
\newtheorem{openproblem}[standardglobalcounter]{Open Problem}
\newtheorem{problem}{Problem}

\theoremstyle{definition}

\newtheorem{property}[standardlocalcounter]{Property}
\newtheorem{definition}[standardlocalcounter]{Definition}
\newtheorem{claim}[standardlocalcounter]{Claim}

\theoremstyle{remark}
\newtheorem{remark}[standardlocalcounter]{Remark}
\newtheorem{example}[standardlocalcounter]{Example}


%
% STUFF FOR ``META-KIND'' OF INTERNAL NOTES --- OBSOLETE 
%

% META COMMENT
\newtheoremstyle{meta}% name
  {3pt}%      Space above
  {3pt}%      Space below
  {\scshape \small }%         Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\scshape \small }% Thm head font
  {:}%        Punctuation after thm head
  { }%     Space after thm head: " " = normal interword space;
        %       \newline = linebreak
  {}%         Thm head spec (can be left empty, meaning `normal')

\theoremstyle{meta}
\newtheorem{meta}{Meta comment}

% OPEN QUESTIONS (IN META COMMENT STYLE INTENDED FOR PRIVATE NOTES)
\newtheoremstyle{questions}% name
  {3pt}%      Space above
  {3pt}%      Space below
  {\sffamily \slshape}%         Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries \sffamily \slshape}% Thm head font
  {:}%        Punctuation after thm head
  { }%     Space after thm head: " " = normal interword space;
        %       \newline = linebreak
  {}%         Thm head spec (can be left empty, meaning `normal')

\theoremstyle{questions}
\newtheorem{questions}{Open questions}




==> doctypedetection.tex <==
%
% DETECTION OF DOCUMENT TYPE
%----------------------------
%
% Version date: March 15, 2010
%
%
% This file needs to be included or inputted so that the conditional
% macro definitions in e.g. the files definitions.tex,
% notationProofComplexity.tex, and notationClauseSpacePebbling.tex 
% will not generate compilation errors for LaTeX.
%

%
% (1)  \conference is used (rightly or wrongly) to detect poster file.
% 
% (2)  \affaddr is used (rightly or wrongly) to detect STOC file.
%     
% (3)  \affiliation and \Section} are used (rightly or wrongly) to detect 
%      FOCS file.
%     
% (4)  \conference is used (rightly or wrongly) to detect poster file.
%     
% (5)  \sicomp is used to detect SIAM journal file.
%     
% (6)  \tnotetext and \ead are used to detect Elsevier journal file.
%     
% (7)  The combination of \journal, \volume, \issue, \copyrightowner, \pubyear,
%      and \articletitle is used (rightly or wrongly) to detect NOW publishers
%      Foundations & Trends.
%     
% (8)  The combination of \keywords, \subjclass, \titlecomment, \revisionname,
%      and \lmcsheading is used (rightly or wrongly) to detect the LMCS style
%      file.
%     
% (9)  The combination of \IEEEtransversionmajor, \IEEEtransversionminor, 
%      \IEEEitemize, \IEEEenumerate, and \IEEEdescription is used (rightly
%      or wrongly) to detect IEEE style file (for CCC)
%     
% (10) If \chapter is not defined, maybeArticle is set to true.
%     
% (11) maybeThesis detects some kthesis-specific macros.
%     
% (12) maybeReport is set to true if neither maybeArticle nor maybeThesis 
%      is true.
%     
%    
% Detection of LLNCS is not implemented.
% 
%
% Use the file 'testdoctypedetection.tex' to test if these
% Boolean detectors work.
%

\usepackage{ifthen}

\newboolean{maybeSTOC}
\newboolean{maybeFOCS}
\newboolean{maybeElsevier}
\newboolean{maybeNOW}
\newboolean{maybeLMCS}
\newboolean{maybePoster}
\newboolean{maybeSIAM}
\newboolean{maybeIEEE}
\newboolean{maybeArticle}
\newboolean{maybeReport}
\newboolean{maybeThesis}

\ifthenelse{\isundefined{\affaddr}}        
{\setboolean{maybeSTOC}{false}}
{\setboolean{maybeSTOC}{true}}

\ifthenelse{\not \isundefined{\affiliation}
  \and \not \isundefined{\Section}}        
{\setboolean{maybeFOCS}{true}}
{\setboolean{maybeFOCS}{false}}

\ifthenelse{\not \isundefined{\tnotetext}
  \and \not \isundefined{\ead}}        
{\setboolean{maybeElsevier}{true}}
{\setboolean{maybeElsevier}{false}}

\ifthenelse{\not \isundefined{\journal} \and 
  \not \isundefined{\volume} \and 
  \not \isundefined{\issue} \and 
  \not \isundefined{\copyrightowner} \and 
  \not \isundefined{\articletitle} \and 
  \not \isundefined{\pubyear}}
{\setboolean{maybeNOW}{true}}
{\setboolean{maybeNOW}{false}}

\ifthenelse{\not \isundefined{\keywords} \and
  \not \isundefined{\subjclass} \and
  \not \isundefined{\titlecomment} \and
  \not \isundefined{\revisionname} \and
  \not \isundefined{\lmcsheading}}
{\setboolean{maybeLMCS}{true}}
{\setboolean{maybeLMCS}{false}}

\ifthenelse{\not \isundefined{\IEEEtransversionmajor} \and 
  \not \isundefined{\IEEEtransversionminor} \and 
  \not \isundefined{\IEEEitemize} \and 
  \not \isundefined{\IEEEenumerate} \and 
  \not \isundefined{\IEEEdescription}}
{\setboolean{maybeIEEE}{true}}
{\setboolean{maybeIEEE}{false}}

\ifthenelse{\isundefined{\sicomp}}
{\setboolean{maybeSIAM}{false}}
{\setboolean{maybeSIAM}{true}}

\ifthenelse{\isundefined{\conference}}
{\setboolean{maybePoster}{false}}
{\setboolean{maybePoster}{true}}

\ifthenelse{\isundefined{\chapter}}
{\setboolean{maybeArticle}{true}}
{\setboolean{maybeArticle}{false}}

\ifthenelse{\not \isundefined{\examen} 
  \and \not \isundefined{\disputationsdatum} 
  \and \not \isundefined{\disputationslokal}}   
  {\setboolean{maybeThesis}{true}}
  {\setboolean{maybeThesis}{false}}
           
\ifthenelse{\boolean{maybeArticle} \or \boolean{maybeThesis}}      
{\setboolean{maybeReport}{false}}
{\setboolean{maybeReport}{true}}



==> notationMatroids.tex <==
%
% FILE WITH SOME MATROID FREENESS LaTeX STUFF THAT MIGHT COME IN HANDY
%

\theoremstyle{plain}    

% This "question" environment can probably be removed in the final version
\newtheorem{question}[standardlocalcounter]{Question}


% NEW MACROS AUG 21 TO GET CONSISTENT (AND NON-OVERLOADED) NOTATION

% Matroids M and N and their labels sigma and tau
\newcommand{\mtrdM}{M}
\newcommand{\mtrdN}{N} 
\newcommand{\mtrdF}{F} 
\newcommand{\mlblS}{\sigma} 
\newcommand{\mlblT}{\tau} 

% Graphic matroid (not consistently used in paper yet -- Aug 23, 2010)
\newcommand{\gmtrd}[1]{\mtrdM({#1})} 

% Set of matroid constraints
\newcommand{\mtrdset}{\mathbb{M}}

% Properties A, B, P, Q and F
\newcommand{\propA}{{\cal A}}
\newcommand{\propB}{{\cal B}}
\newcommand{\propP}{{\cal P}}
\newcommand{\propQ}{{\cal Q}}
\newcommand{\propF}{{\cal F}}

% Function domain and range
\newcommand{\fdomain}{{\cal D}}
\newcommand{\frange}{{\cal R}}

% Notation for matroid embeddings
\newcommand{\membeds}{\hookrightarrow}
\newcommand{\notmembeds}{\not\hookrightarrow}

% Notation for weight of vectors
\newcommand{\weight}[1]{\lvert{#1}\rvert}
\newcommand{\vecweight}[1]{\weight{\matroidvector{#1}}}

% Short-hand for matroid vectors
\newcommand{\matroidvector}[1]{\vec{#1}}
\renewcommand{\matroidvector}[1]{\mathbf{#1}}
\newcommand{\vecb}{\matroidvector{b}}
\newcommand{\vece}{\matroidvector{e}}
\newcommand{\vecf}{\matroidvector{f}}
\newcommand{\vecu}{\matroidvector{u}}
\newcommand{\vecv}{\matroidvector{v}}
\newcommand{\vecw}{\matroidvector{w}}
\newcommand{\vecx}{\matroidvector{x}}
\newcommand{\vecy}{\matroidvector{y}}
\newcommand{\vecz}{\matroidvector{z}}
\newcommand{\veczero}{\matroidvector{0}}

% Notation for fields K and F
\newcommand{\K}{\mathbb{K}}
\newcommand{\F}{\mathbb{F}}

% Notation for patterns (with angle brackets)
\newcommand{\pattern}[1]{\langle {#1} \rangle}
\newcommand{\patternindexed}[2]{\langle {#1} \mid {#2} \rangle}

% Notation for the canonical function for a labelled matroid
%\newcommand{\jset}{\mathbf{j}}
\newcommand{\jset}{J}
\newcommand{\jproj}[2][\jset]{{#2}[{#1}]}
\newcommand{\jprojv}[2][\jset]{\matroidvector{#2}[#1]}
\newcommand{\jcomp}[2]{\{{#1}|{#2}\}}
\newcommand{\jcompv}[2]{\jcomp{\matroidvector{#1}}{\matroidvector{#2}}}
  
%\canonfunc{matroid}{pattern}{padding bit}
%    \newcommand{\canonfunc}[3]{f^{#3}_{{#1},{#2}}}
\newcommand{\canonfunc}[3]{f^{#3}_{#1,#2}}
\newcommand{\canonfuncstd}{\canonfunc{N}{T}{b}}

% Calligraphic A,B,P (for properties), T (for transformations),
% and S (for sets of patterns)
\newcommand{\cala}{{\cal A}}
\newcommand{\calb}{{\cal B}}
\newcommand{\calp}{{\cal P}}
\newcommand{\cals}{{\cal S}}
\newcommand{\calt}{{\cal T}}

% Some other cal:s
\newcommand{\calf}{\mathcal{F}}
\newcommand{\calm}{\mathcal{M}}
\newcommand{\caln}{\mathcal{N}}



\newcommand{\supp}[1]{\mathrm{supp}(#1)}

%%% Ning's macros
\newcommand{\ignore}[1]{}
\newcommand{\rednote}[1]
%  {}
{\textcolor{red}{#1}}
\newcommand{\bluenote}[1]
%  {}
{\textcolor{blue}{#1}}
\newcommand{\eps}{\epsilon}
%    \newcommand{\eqdef}{{\stackrel{\rm def}{=}}}

%    \newcommand{\sidenote}[1]%
%    {\leavevmode\marginpar{\raggedright\footnotesize\sffamily #1}\ignorespaces}

\newcommand{\sidenote}[1]{\editcomment{#1}}

\renewcommand{\sidenote}[1]{\editcomment{\textcolor{red}{#1}}}

%    
%    \newcommand{\sidenote}[1]{ \marginpar{\tiny\bf
%                 \begin{minipage}[t]{0.5in}
%                   \raggedright #1
%                \end{minipage}}}
%    



